A meta-algorithm for classification using random recursive tree ensembles: A high energy physics application

The aim of this work is to propose a meta-algorithm for automatic classification in the presence of discrete binary classes. Classifier learning in the presence of overlapping class distributions is a challenging problem in machine learning. Overlapping classes are described by the presence of ambiguous areas in the feature space with a high density of points belonging to both classes. This often occurs in real-world datasets, one such example is numeric data denoting properties of particle decays derived from high-energy accelerators like the Large Hadron Collider (LHC). A significant body of research targeting the class overlap problem use ensemble classifiers to boost the performance of algorithms by using them iteratively in multiple stages or using multiple copies of the same model on different subsets of the input training data. The former is called boosting and the latter is called bagging. The algorithm proposed in this thesis targets a challenging classification problem in high energy physics - that of improving the statistical significance of the Higgs discovery. The underlying dataset used to train the algorithm is experimental data built from the official ATLAS full-detector simulation with Higgs events (signal) mixed with different background events (background) that closely mimic the statistical properties of the signal generating class overlap. The algorithm proposed is a variant of the classical boosted decision tree which is known to be one of the most successful analysis techniques in experimental physics. The algorithm utilizes a unified framework that combines two meta-learning techniques - bagging and boosting. The results show that this combination only works in the presence of a randomization trick in the base learners.

==> chapters/kaggle.tex <==
The Higgs Machine learning challenge (HiggsML for short) hosted on Kaggle and sponsored by ATLAS attracted unprecedented interest from scientists in various different fields including physicists. Over 6000 people downloaded the data and by the end of the competition had uploaded over 35000 solutions among 1785 teams \cite{postRM}. The scores of all the teams are publicly available on the leader board of the HiggsML challenge on the Kaggle platform at \url{https://www.kaggle.com/c/higgs-boson/leaderboard}.

The Higgs classification problem is unique in the sense that goal of the challenge is not just to discriminate between Higgs and non-Higgs events but to provide a solution that maximizes a peculiar significance metric called the AMS ($\sigma$) based on the selection of a signal-rich region of the high-dimensional feature space. There was considerable mathematical nuance surrounding the physics of the problem. The organizers provided a training set to participants with 250K labelled events and provided an unlabelled set of 550K test events for participants to provide predictions for. The organizers reserved the weights and labels for the test events in order to prevent teams from over-fitting to the test set.  

The winning solution with the highest reported score was by Gabor Melis, a professional data scientist from Hungary. The AMS value of his solution was 3.80581. His model was an ensemble of multi-layer neural networks which used the principle of bagging. Each neural network was trained on a different subset of the full dataset creating a heterogeneous mix of networks. The output of each model was a probability estimate (usually, it is the probability that a given event belongs to the positive signal class). The prediction on an unseen sample used simple arithmetic averaging to combine the probability outputs of the bag of  models. In his own words, the most important characteristic of his model was incorporating a careful bagging procedure. His solution reflects the power of the split-train-recombine technique. Gabor published a summary account of his methodology in \cite{melis}. 

The second place winner Tim Salimans achieved a AMS score of 3.78913 on the leader board. He used a regularized greedy forest which is a variant on gradient boosting and pushes trees further away from greedy construction by adding explicit regularization terms \cite{rgf}. Further, he added and additional 30 features to the dataset taking the training time to several hours on a 4-core CPU.

XGBoost \cite{xgb} was one of the most popular choices among participants, it was rated the best single model to give strong results on the Higgs dataset. The model was used by roughly 25$\%$ of the participants and set a high performance benchmark in terms of score and speed. XGBoost is a highly scalable version of a gradient tree boosting algorithm and is available as an open source package. Part of its popularity was attributed to the fact that it provided a 10x speed scale up to the standard gradient boosting algorithm provided in python \texttt{scikit-learn}. It does so by proposing an approximate algorithm to the greedy tree construction algorithm. However, the best XGBoost model score was not in the top $10\%$ of scores achieved by participants. Many of the participants used XGBoost as part of larger ensembles with different algorithms in the mix and achieved higher scores than the single XGBoost model. This goes to show that while XGBoost is a powerful model, there was room for improving performance using different types of ensembles.  

The one thing that is apparent from this study is that a lot of the models that bagged top scores were overkill in terms of their architecture and computational sophistication. Gabor Melis trained his ensemble of neural networks on a GTX Titan GPU where training a single 3-layer network took 10 minutes. As a comparison the solution provided in this thesis runs on a 4-core CPU machine and the entire model trains in under 30 mins. The winning scores are in table \ref{leader}, the boosted extremely random trees (BXT) algorithm proposed in this thesis achieves an AMS score of 3.793$\sigma$. 

\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{images/leaderboard_final.jpg}
\caption{Leading solutions to the HiggsML Challenge (2014)}
\label{leader}
\end{figure}



==> chapters/litreview.tex <==


The content of this section summarises the most significant published approaches in, 

\begin{itemize}
\item The most successful applications of machine learning in high energy physics problems. 
\item Primary machine learning research targeted to the problem of overlapping class distributions in context of high dimensional data. 
\end{itemize}

It addresses a specific gap in the current methods being used to tackle classification problems with significant class overlap. 

==> chapters/meta.tex <==




==> chapters/overlap.tex <==
%\section{Recap of the problem}
%\label{mlc}
%
%The machine learning aim of this thesis is to explore the statistical challenges in classifying signal (higgs events) from background (non-higgs events). In constructing a classifier for this problem one needs to address the main sources of complexity in the data. They arise from overlap and imbalance.
%
%Both the signal and background events in the data have the same decay signature with the only discriminating feature being the subtle differences in the measured properties of their decay products.
%
%The signal events represent collisions where the parent Higgs was created and background events represent collisions where the parent particle was not Higgs but shared the same tau-tau decay channel. Neutrinos created in the collisions escape detection and the only feature hinting at their properties is the missing transverse momentum explained in section \ref{missing} of Chapter \ref{intro}. In the rest of the thesis, the following terminology is applied.
%
%\begin{enumerate}
%\item Signal event: An event in which a Higgs decays to a pair of tau leptons. In machine learning vocabulary, a signal is a member of the positive class.
%\item Background event:  An event in which a non-Higgs decay process occurs. In machine learning vocabulary, a background event is a member of the negative class. 
%\item Selection Region: A classifier outputs a score or a discriminant value $f(\textbf{x})$ which is a score taking small values for the negative class and large values for the positive class. The selection region is defined by applying a threshold of choice $\theta$ on $f(\textbf{x})$ and selecting all the events that lie above the threshold.
%\end{enumerate}
%
%From a machine learning perspective, a classifier in this context has to tackle the following challenges:
%
%\begin{enumerate}
%\item The classes completely overlap, the signal and background events appear coalesced when visualized for different features. 
%\item The discovery significance metric AMS ($\sigma$) is unusual and not a function of classification accuracy. 
%\item The classifier in this context is used as a selection method which defines a region in the feature space rich in signal events. The data consists of 30 features. 
%\item The AMS metric is prone to over-fitting as the value of the AMS depends upon a small number of events selected as signal by the classifier. 
%\item The AMS is noisy and not conducive to direct optimization, instead a classifier is designed to optimize a machine learning metric which closely reflects the AMS. 
%\end{enumerate}


%The use of standard machine learning performance metrics like accuracy and error rate are rendered misleading in the presence of imbalanced classes. For instance, it is straightforward to achieve an accuracy of 75\% in a domain where the majority class corresponds to 75\% of the instances. 

In class imbalance problems the minority class is usually of primary interest .i.e., the error costs are not uniform across both classes. For instance, it might be more critical to detect as many of the positive class instances correctly than to miss-classify some of the instances of the negative class. This is usually the case in real-world applications with majority-minority class distributions. The costs of classifying a sick person as healthy is far greater than classifying some healthy persons as sick. In such cases the false negative rate is a far more critical measure of performance than the false positive rate.

In the Higgs problem where we are trying to classify signal from background, we have established that the AMS ($\sigma$) is far more sensitive to the presence of background events in the selection region (false positives) and is less sensitive to the signals dropped off in the rejection region. What matters is the purity of events in the selection region, this is affected more by false positives than by false negatives. 

%\section{Complexity in binary classification}
%
%While class overlap may occur in classification problems, the fact that they arise from two  different underlying distributions should leave hidden markers to differentiate them. Data from two non-random underlying distributions is different to data that has been randomly labelled even if the former completely overlap. In this section we discuss some measures that characterize the difficulty of a classification problem in the presence of overlap \cite{hobasu}. Measures that quantify the difficulty of classifying at the dataset level and at the data point level can provide avenues for meta-learning.  
%
%\begin{enumerate}
%
%\item Fisher's discriminant ratio (F1): 
%It is defined as, 
%\begin{equation}
%f = \frac{(\mu_{1} - \mu_{2})^2}{\sigma_{1}^{2} + \sigma_{2}^{2}}
%\end{equation}
%where $\mu_{1}$, $\mu_{2}$, $\sigma_{1}^{2}$, $\sigma_{2}^2$ are the means and variances of the two classes for a particular feature is a measure of how the respective feature contributes to class discrimination.  
%
%\item Tomek links:  Given a dataset $\mathbf{D} = \{(\mathbf{x}_{1},y_{1}) \ldots (\mathbf{x}_{n},y_{n})\}$ where each $\mathbf{x}_{i} \in \mathbb{R}^d$ and $d > 1$, a pair of points $(\mathbf{x}_{i}, \mathbf{x}_{j})_{i \neq j}$ has a tomek link if $d(\mathbf{x}_{i}, \mathbf{x}_{j}) < d(\mathbf{x}_{i}, \mathbf{x}_{k})$ $\forall k \in n$ and $y_{i} \neq y_{j}$, $d$ is a distance metric. In other words if the nearest neighbour of a data point is a member of a different class then a tomek links exists between the two points. Detecting and removing tomek links from the training dataset is a method of de-noising the data and can many times boost classification performance and give smoother decision boundaries.   
%
%Detection of tomek links when each data point has several dimensions is a non-trivial problem, it essentially amounts to search in a high dimensional space. A naive implementation has a complexity of $\mathcal{O}(n^{2})$.
%
%\end{enumerate} 


